RangeSeg: Range-Aware Real Time Segmentation of 3D LiDAR Point Clouds

Semantic outdoor scene understanding based on 3D LiDAR point clouds is a challenging task for autonomous driving due to the sparse and irregular data structure. This paper takes advantages of the uneven range distribution of different LiDAR laser beams to propose a range aware instance segmentation network, RangeSeg. RangeSeg uses a shared encoder backbone with two range dependent decoders. A heavy decoder only computes top of a range image where the far and small objects locate to improve small object detection accuracy, and a light decoder computes whole range image for low computational cost. The results are further clustered by the DBSCAN method with a resolution weighted distance function to get instance-level segmentation results. Experiments on the KITTI dataset show that RangeSeg outperforms the state-of-the-art semantic segmentation methods with enormous speedup and improves the instance-level segmentation performance on small and far objects. The whole RangeSeg pipeline meets the real time requirement on NVIDIA\textsuperscript{\textregistered} JETSON AGX Xavier with 19 frames per second in average.

==> fig/encoding.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=!,width=0.4\linewidth,keepaspectratio=true]%
    {figures/RVencoding}
    \caption{The spherical coordinate of the range image encoding.  $\theta$ and $\phi$ are an azimuth angle and an elevation angle.  $r$ is the range of the point.  A 3D point $(x,y,z)$ can be encoded into $(r,\theta,\phi)$ through this spherical coordinate system.}
    \label{fig:RVencoding}
\end{figure}

==> fig/heavydecoder-arch.tex <==
\begin{figure}[t]
    \centering
    \subfloat[Up-sample modules]{
        \includegraphics[height=!,width=0.5\linewidth,keepaspectratio=true]%
    {figures/heavydecoder-detail}
    \label{fig:heavydecoder-detail}
    }
    \subfloat[Dense DLA]{
        \includegraphics[height=!,width=0.5\linewidth,keepaspectratio=true]%
    {figures/heavydecoder-arch-v2}
    \label{fig:densDLA}
    }
    \caption{The architecture of the heavy decoder.  The orange boxes in (b) are up-sample modules whose detail are plotted in (a) and the blue boxes are normal feature extractors.}
    \label{fig:heavydecoder-arch}
\end{figure}

==> fig/heavydecoder-arch_new.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=!,width=\linewidth,keepaspectratio=true]%
    {figures/heavydecoder-arch_new}
    \caption{The architecture of the heavy decoder.  The blue block is the feature extractor and the orange block is the up-sample module.  The details of the up-sample module are shown on the left part.}
    \label{fig:RVencoding}
\end{figure}

==> fig/heavydecoder-arch_new_v2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=!,width=\linewidth,keepaspectratio=true]%
    {figures/heavydecoder-arch_new_v2}
    \caption{The architecture of the heavy decoder.  The blue block is the feature extractor and the orange block is the up-sample module.  The black arrow denotes the down-sample of feature extractors.  The blue one denotes the input of DeConv.  The green one denotes the no. The details of up-sample module are shown on the left part.}
    \label{fig:RVencoding}
\end{figure}

==> fig/lightdecoder-arch.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=!,width=0.7\linewidth,keepaspectratio=true]%
    {figures/lightdecoder-detail}
    \caption{The architecture of the light decoder.}
    \label{fig:lightdecoder-arch}
\end{figure}

==> fig/lightdecoder-arch_new.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=!,width=\linewidth,keepaspectratio=true]%
    {figures/lightdecoder-arch_new}
    \caption{The architecture of the light decoder.  The blue block is the feature extractor and the orange block is the up-sample module.  The details of up-sample module are shown on the left part.}
    \label{fig:RVencoding}
\end{figure}

==> fig/superconvergence.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=!,width=\linewidth,keepaspectratio=true]%
    {figures/sc}
    \caption{The curve of how super convergence changes the learning rate every iteration.  The target learning rate in the figure is 0.1.  The initial learning rate 0.01 will increase to the target learning rate 0.1 in the first 450 iterations.  The learning rate will start decreasing to 0.01 after $450^{th}$ iteration.  The learning rate will continue decreasing in the last 100 iterations.}
    \label{fig:superconvergence}
\end{figure}

==> table/ablation-loss.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ c c }
        \toprule
        Loss & mIoU(\% ) \\
        \midrule
        xent & 45.8 \\
        focal & 20.6 \\
        lov\'{a}sz & 39.6 \\
        focal+lov\'{a}sz & 56.7 \\
        xent+lov\'{a}sz & \textbf{59.1} \\
        \bottomrule
    \end{tabular}
    \caption{Ablation study on the loss function.}
    \label{table:ablation-loss}
\end{table} 

==> table/ablation-pre.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ c c }
        \toprule
        Data Pre-processing & mIoU(\% ) \\
        \midrule
        Norm. & 59.8\\
        Norm. w/ Aug. & \textbf{63.2} \\
        \bottomrule
    \end{tabular}
    \caption{Ablation study on data pre-processing.}
    \label{table:ablation-pre}
\end{table} 

==> table/ablation-scale.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ c c }
        \toprule
        Scale loss & mIoU(\% ) \\
        \midrule
        w/o scale loss & 62.0 \\
        w/ scale loss & \textbf{65.9} \\
        \bottomrule
    \end{tabular}
    \caption{Ablation study on the range-aware framework.}
    \label{table:ablation-scale}
\end{table}

==> table/kitti3d-fps.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{ c  >{\centering\arraybackslash}m{1.2cm}  >{\centering\arraybackslash}m{1.5cm}  >{\centering\arraybackslash}m{1.5cm} >{\centering\arraybackslash}m{1.5cm} }
        \toprule
        {Architecture} & FPS & FLOPs(G) &  mIoU(\% )  \\
        \toprule
        UNet & 249.8 & 15.59 &  63.3  \\
        \midrule
        ResNet18-UNet & \textbf{122.9} & \textbf{44.25} &  62.0 \\
        ResNet34-UNet & 76.6 & 79.34 & 65.6 \\
        Ours(ResNet18) & 89.2 & 56.16 & \textbf{65.9} \\
        \midrule
        LaserNet-DLA & 77.0 & 62.60 & 66.0 \\
        Ours(LaserNet) & \textbf{109.1} & \textbf{39.84} & \textbf{67.9} \\
        \bottomrule
    \end{tabular}
    \caption[FPS, FLOPs, the number of parameters comparison.]{FPS, FLOPs, the number of parameters comparison.}
    \label{table:kitti3d-fps}
\end{table} 
